CLiC: Concept Learning in Context

This paper addresses the challenge of learning a local visual pattern of an object from one image, and generating images depicting objects with that pattern. Learning a localized concept and placing it on an object in a target image is a nontrivial task, as the objects may have different orientations and shapes. Our approach builds upon recent advancements in visual concept learning. It involves acquiring a visual concept (e.g., an ornament) from a source image and subsequently applying it to an object (e.g., a chair) in a target image. Our key idea is to perform in-context concept learning, acquiring the local visual concept within the broader context of the objects they belong to. To localize the concept learning, we employ soft masks that contain both the concept within the mask and the surrounding image area. We demonstrate our approach through object generation within an image, showcasing plausible embedding of in-context learned concepts. We also introduce methods for directing acquired concepts to specific locations within target images, employing cross-attention mechanisms, and establishing correspondences between source and target objects. The effectiveness of our method is demonstrated through quantitative and qualitative experiments, along with comparisons against baseline techniques.

==> sec/intro_old.tex <==
\section{Introduction}
\label{sec:intro}
\am{All objects around us are decorated with geometric ornaments and aesthetical patches. Such decorations and artifacts make objects around us unique, creative, and aesthetically pleasing. Realizing such geometric patterns, detecting them and remixing them with other objects have great value in design, architecture, art, etc. However, detecting geometric ornaments and aesthetics is a difficult task due to the lack of ground truth and subjectivity of the problem. More importantly, transferring such artifacts from one object to another is not an easy task since the new source and target shapes might be from different categories, in different sizes, and in different styles.}

\am{Naively changing the style of a shape or simple copy and pate of ornaments results in modifying the entire object losing the original structural and stylistic characteristic of the object (see Figure). Instead, we want to be able to transfer ornaments and aesthetics to a target shape while the overall shape is not affected by drastic and unwanted modifications (see Figure). In fact, we are looking for a \emph{controllable} mechanism to borrow ornaments or styles from one shape to another. For example, looking at Figure \ref{}, we intend to change the pillars of the building into the style of the source while keeping the rest of the building intact. Also, the pillars should be seamlessly blended into the target image therefore a simple copy-and-paste approach will not be effective. }\ali{Mehdi, add the necessary figures. Also a teaser.}

\am{There have been attempts to change the style of an image \cite{} or composition a patch into another image \cite{}. However, these approaches are unable to effectively perform the task of \emph{geometric ornament transform} as they either heavily modify the target shape or the desired ornaments or patches that are supposed to be transferred.} \am{Textual inversion learns a token for a global shape from multiple images. It is unable to properly learns a token from a single image for a local object or region. Break a scene localizes the objects within a scene by utilizing a series of masks that contain the objects. However, break a scene does not learn a token that is context aware. Meaning that if we learn a token for a patch located on a chair, the token learned by break a scene is not aware of the relation of that patch with the chair. This results in unwanted texture, size, and location mismatch when the patch is transferred to another object. However, in our work by learning a context-aware local token, we are able to successfully synthesize the concept learned from a local region on a target shape.}

\am{To perform this task, we utilize diffusion models. Given a source image, we intend to transfer patches of the source image to a target image in a seamless manner. First, the desired patches on the source image are learned or annotated. Then the corresponding regions of those patches on the target shapes are learned through an optimization of the attentions of a pre-trained diffusion model. Then, a token representing that style is learned and the patches are transferred to the target shape with a proper text prompt and multiple losses that guarantee a smooth ornament transfer from the source to the target (see Section \ref{}).} \ali{Mehdi, make sure my explanation is correct. Try to add more content about the losses. }

\am{Our contributions are as follows:} \ali{add the contributions.}


\am{Through multiple quantitative and qualitative comparisons, we have shown the efficacy of our approach. As apparent in the results (see Figure \ref{}), no other previous work is capable of transferring geometric ornaments seamlessly without drastically changing the target shape. }
